A shape derivative approach to domain simplification

The objective of this study is to address the difficulty of simplifying the geometric model in which a differential problem is formulated, also called defeaturing, while simultaneously ensuring that the accuracy of the solution is maintained under control. This enables faster and more efficient simulations, without sacrificing accuracy. More precisely, we consider an isogeometric discretisation of an elliptic model problem defined on a two-dimensional hierarchical B-spline computational domain with a complex boundary. Starting with an oversimplification of the geometry, we build a goal-oriented adaptive strategy that adaptively reintroduces continuous geometrical features in regions where the analysis suggests a large impact on the quantity of interest. This strategy is driven by an a posteriori estimator of the defeaturing error based on first-order shape sensitivity analysis, and it profits from the local refinement properties of hierarchical B-splines. The adaptive algorithm is described together with a procedure to generate (partially) simplified hierarchical B-spline geometrical domains. Numerical experiments are presented to illustrate the proposed strategy and its limitations.

==> algorithm_backup.tex <==
%\textcolor{red}{\begin{itemize}
%\item add simple picture to explain
%\end{itemize}}

\noindent This section proposes an adaptive algorithm aimed at constructing a simplified geometry $\Omega_S$ that yields a sufficiently accurate value of the functional of interest $\mathcal{J}(\cdot)$, i.e. such that  
\begin{align}
\label{eq:convergence_criterion}
    \abs{\mathcal{J}(\Omega) - \mathcal{J}(\Omega_S)} < \varepsilon
\end{align}
for a given tolerance $\varepsilon$.\\
% \noindent Let us start by commenting on its name, to highlight its main features. 
\noindent As in any other \emph{adaptive} framework, we devised an iterative strategy to build increasingly detailed geometries based on the following steps:
\begin{center}
    SOLVE $\rightarrow$ ESTIMATE $\rightarrow$ MARK $\rightarrow$ REFINE.
\end{center}
\noindent In our context, the SOLVE step corresponds to the computation of the functional $\mathcal{J}(\cdot)$ on the geometry $\Omega_n$ at the current iteration $n$, while the ESTIMATE step corresponds to the estimation of the modelling error~\eqref{eq:modelling_err}. Regarding the last two steps, rather than directly selecting a set of local features to create the refined geometry $\Omega_{n+1}$, we construct a locally refined THB-spline space to represent it. Hence, we choose a suitable set of basis functions in the MARK step, while the REFINE step enriches the given THB-spline space starting from this set to increase the complexity of the geometry.  \\
\noindent Our algorithm is \emph{gradient based} for two reasons: on the one side, the marking and refinement procedures rely on the evaluation of the (first order) sensitivity of the functional at hand to a modification of the domain (see Subsections~\ref{subsec:algo_mark} and \ref{subsec:algo_refine}); on the other, our heuristic estimator for the modelling error is also defined through the same values of the first order sensitivities (see Subsection~\ref{subsec:algo_estimate}). \\

\noindent To illustrate the algorithm, we fully describe one of the iterations that allow us to construct the final simplified domain $\Omega_S$ starting from the simplest possible geometry $\Omega_0$ for the problem at hand. The main steps are then summarised in Algorithm~\ref{algo:simplification}. \\
We consider the iteration $n$, where the hierarchical mesh $\mathcal{Q}_n$ and the associated THB-spline space generated by $\mathcal{T}_n$, with cardinality $\dim(\mathcal{T}_N) := N_n$ describe the geometry $\Omega_n$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Solve}\label{subsec:algo_solve}
In this step, we compute the value of the functional $\mathcal{J}(\Omega_n)$ after solving the state problem~\eqref{eq:weak_state_pb} on $\Omega_n$. Moreover, we also solve the adjoint problem~\eqref{eq:weak_adj_pb} on the same geometry, as its solution is needed for the computation of the shape derivatives as explained in Section~\ref{subsec:shapeder}.\\
\noindent Since the main focus of this work concerns the \textcolor{red}{modelling error}, for the moment we assume that an exact solution of the PDE problem is available on both the simplified and the exact geometry. In other words, we disregard the error due to the numerical approximation of the PDE problems. The issue of taking into account this error in the isogeometric setting will be briefly addressed by the numerical experiments in Section \ref{sec:numerical}.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Estimate}\label{subsec:algo_estimate}
To achieve our goal of controlling the \textcolor{red}{modelling error} on simplified geometries, we must introduce a suitably computable estimator of the error~\eqref{eq:modelling_err} that we use as a stopping criterion of our iterative algorithm. As mentioned before, our choice is based on the first order shape derivatives of $\mathcal{J}$: indeed, given a finite set $\Theta_n$ of directions $\bm{\theta}_k$ as in Definition~\ref{def:direct_shapeder}, we define the error estimator as
\begin{equation}
\label{eq:estimator}
E_n^{\text{mod}}(\Omega_n) \vcentcolon = \max_{\bm{\theta}_k \in \Theta_n} \, \bigg |\frac{\operatorname{d}\! \mathcal{J}}{\operatorname{d} \!\Omega}\Big(\Omega_n\, \Big|\, \bm{\theta}_k\Big) \bigg|.
\end{equation}
The numerical experiments show that, by choosing $\Theta_n$ wisely (as detailed in the next Subsection~\ref{subsec:algo_mark}), this quantity is a good estimator of the modelling error, although a proof of its reliability and efficiency goes beyond the scope of this work.
%The numerical experiments show that this heuristic estimator provides a good upper bound for the modelling error, although a proof of its reliability and efficiency goes beyond the scope of this work.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mark}\label{subsec:algo_mark}
This section illustrates the core of our algorithm, that is, approximating the exact boundary correspondence $\mathbf{F}: \partial \widehat{\Omega} \rightarrow \partial \Omega$, picking the directions of differentiation $\bm{\theta}_k$ and employing the estimator~\eqref{eq:estimator} in the marking process.\\

\noindent Given the current iteration's THB-spline basis \smash{$\mathcal{T}_n = \{\beta_i \}_{i=1}^{N_n}$}, the first step approximates the exact boundary $\partial \Omega$ over the subset $\widetilde{\mathcal{T}}_n \subset \mathcal{T}_n$ with cardinality $\dim ( \widetilde{\mathcal{T}}_n ) := \partial N_{n}$ comprised of all $\beta_i \in \mathcal{T}_n$ that do not vanish on the boundary. We accomplish this by fitting the set of boundary control points \smash{$\partial \mathcal{C} = \{\mathbf{c}_i \}_{i=1}^{\partial N_n}$} via a scaled $H^1(\partial \widehat{\Omega})$ projection. To be precise, the fitting routine selects $\partial \mathcal{C}$ such that
\begin{align}
\label{eq:boundary_fit}
    & \kappa_0 \int \limits_{\partial \widehat{\Omega}} \left \| \mathbf{F}_n - \mathbf{F} \right \|^2 \operatorname{d}\!x + \kappa_1 \int \limits_{\partial \widehat{\Omega}} \left \| \frac{\partial(\mathbf{F}_n - \mathbf{F})}{\partial t} \right \|^2 \operatorname{d}\!x \longrightarrow \min \limits_{\partial \mathcal{C}},
\end{align}
wherein \smash{$\tfrac{\partial}{\partial t}(\, \cdot \,)$} denotes the directional derivative along the unit tangent of $\partial \widehat{\Omega}$, while $\kappa_0 > 0$ and $\kappa_1 \geq 0$ are constants tuning the magnitude of the $L^2(\partial \widehat{\Omega})$ and $H^1(\partial \widehat{\Omega})$ semi-norms in the fit. The minimisation from (\ref{eq:boundary_fit}) may furthermore be subjected to constraints such as requiring the fit to assume the exact value of $\mathbf{F} \vcentcolon \partial \widehat{\Omega} \rightarrow \partial \Omega$ in the four corners of the parametric domain. \\

\noindent With the resulting set $\partial \mathcal{C}$, this yields the following parameterisation of the boundary $\partial \Omega_n$:
$$ \mathbf{F}_n \vcentcolon \partial \widehat{\Omega} \rightarrow \partial \Omega_n \qquad \text{such that} \qquad \mathbf{F}_n(\bm{\xi}) = \sum_{i=1}^{\partial N_n} \mathbf{c}_{i}\beta_{i}(\bm{\xi}) \qquad \forall  \ \bm{\xi} \in \partial \widehat{\Omega}.$$
Let then $\mathcal{Q}_n^+$ be the hierarchical mesh obtained by dyadic refinement of the boundary elements of $\mathcal{Q}_n$, that is, of those elements $Q \in \mathcal{Q}_n$ with $\partial Q \cap \partial \widehat{\Omega} \neq \emptyset$. By \smash{$\mathcal{T}_n^+ = \{\beta^+_{i}\}_{i=1}^{N_n^+}$} we denote the canonical THB-spline basis associated with $\mathcal{Q}^+_n$. As before, we consider the subset $\widetilde{\mathcal{T}}_n^+ \subset \mathcal{T}_n^+$ of the $\partial N_n^+$ basis functions that do not vanish on $\partial \widehat{\Omega}$.
Thanks to the \emph{two-scale relation}~\eqref{eq:two_scale}, we can express $ \mathbf{F}_n: \partial \widehat{\Omega} \rightarrow \partial \Omega_n$ in terms of this subset:
$$  \mathbf{F}_n(\bm{\xi}) = \sum_{i=1}^{\partial N^+_n} \mathbf{\overline{c}}_{i} \beta^+_{i}(\bm{\xi}) \qquad \forall  \ \bm{\xi} \in \partial \widehat{\Omega}.$$
Our goal is to create a set of THB splines \smash{$\widetilde{\mathcal{T}}_{n+1}$} to express the boundary at the next iteration. To this aim, we choose some of the basis functions in \smash{$\widetilde{\mathcal{T}}_n^+$} according to their impact on the functional of interest, measured in terms of the value of the shape derivative of $\mathcal{J}(\cdot)$ in the corresponding direction. In the following, we only need to clarify how we associate a direction of differentiation $\bm{\theta}_k$ to a basis function.\\

\noindent We accomplish this by minimizing~\eqref{eq:boundary_fit} over the set $\partial \mathcal{C}^+$ of boundary control points associated with $\widetilde{\mathcal{T}}_n^+$ which yields the new fit
$$  \mathbf{F}^+_n \vcentcolon \partial \widehat{\Omega} \rightarrow \partial \Omega^+_n \qquad \text{such that} \qquad \mathbf{F}^+_n(\bm{\xi}) = \sum_{i=1}^{\partial N^+_{n}} \mathbf{c}^+_{i}\beta^+_{i}(\bm{\xi}) \qquad \forall  \ \bm{\xi} \in \partial \widehat{\Omega}.$$

\noindent Since we aim to only select basis functions of $\widetilde{\mathcal{T}}_n^+$ that significantly affect the shape functional $\mathcal{J}(\cdot)$, we evaluate its sensitivity to the perturbations of $\partial\Omega_{n}$ obtained by modifying only one of the control points at a time. To illustrate this idea, let us fix an index $k$ and assume that the boundary control point $\mathbf{\overline{c}}_{k}$ associated to $\beta_k^+$ is changed to $\mathbf{c}^+_{k}$ in the new fit. We can then construct the following mapping of the perturbed boundary $\partial \Omega_{n,k}$:
$$\mathbf{F}_{n,k} \vcentcolon \partial \widehat{\Omega} \rightarrow \partial \Omega_{n,k} \qquad \text{such that} \qquad \mathbf{F}_{n,k}(\bm{\xi}) = \sum_{i\neq k}^{\partial N^+_{n}} \mathbf{\overline{c}}_{i}\beta^+_{i}(\bm{\xi}) + \mathbf{c}^+_{k}\beta^+_{k}(\bm{\xi}) \qquad \forall  \ \bm{\xi} \in \partial \widehat{\Omega},$$
and employ it to define a suitable perturbation map $\mathbf{T}_t^{n,k}$ such that $\mathbf{T}_0^{n,k} (\Omega_n)= \Omega_n$, $\mathbf{T}_1^{n,k} (\Omega_{n})= \Omega_{n,k}$ and 
$$ \mathbf{T}_t^{n,k}\big(\mathbf{F}_n(\bm{\xi})\big) = \mathbf{F}_n(\bm{\xi}) + t\big(\mathbf{F}_{n,k}(\bm{\xi})-\mathbf{F}_n(\bm{\xi})\big) \qquad \forall  \ \bm{\xi} \in \partial \widehat{\Omega}.$$
Recalling Definition~\ref{def:direct_shapeder} of the directional shape derivative requires us to write the restriction to the boundary of such a map in the form $\mathbf{T}_t^{n,k}(\bm{x}) = \bm{x} + t \bm{\theta}_k(\bm{x})$, where $\bm{\theta}_k$ denotes the vector field prescribing the direction of differentiation. Hence, noticing that the parameterization $\mathbf{F}_n$ is invertible, it follows that:
 $$\bm{\theta}_k(\bm{x}) = \mathbf{F}_{n,k}\big(\mathbf{F}^{-1}_n(\bm{x})\big) - \bm{x} = 
 \begin{cases}
 	0, \qquad  \qquad \qquad \qquad \qquad \ \text{if} \  \mathbf{F}^{-1}_n(\bm{x})\notin \left(\overline{\supp{\beta^+_{k}}} \cap \partial \widehat{\Omega} \right)\\
 	( \mathbf{c}^+_{k} - \mathbf{\bar{c}}_{k} )\beta^+_{k}\big(\mathbf{F}^{-1}_n(\bm{x})\big), \qquad  \qquad \qquad \text{otherwise}
 \end{cases}$$
which inherits the regularity of the chosen spline basis and allows us to compute the shape derivative \smash{$\displaystyle \tfrac{\operatorname{d}\! \mathcal{J}}{\operatorname{d} \!\Omega}\left(\Omega_n \, |\, \bm{\theta}_k \right)$} as detailed in Section~\ref{subsec:shapeder}, provided we know the exact solutions $u, p$ of the state problem~\eqref{eq:weak_state_pb} and its adjoint~\eqref{eq:weak_adj_pb} on $\Omega_{n}$. \\
For the purposes of this paper, 

\noindent Following the same reasoning, we compute the shape derivatives associated to all the boundary degrees of freedom and then select only the most significant ones according to a maximum strategy: given a parameter $\alpha \in (0,1)$, the set \smash{$\mathcal{D}^+_{\text{bdry}}  \subset \widetilde{\mathcal{T}}_n^+$} contains all the basis functions $\beta^+_{k}$ such that the associated shape derivative satisfies:
\begin{equation}
\label{eq:selection_criterion}
    \bigg|\frac{\operatorname{d}\! \mathcal{J}}{\operatorname{d} \!\Omega}\Big(\Omega_n\Big|\, \bm{\theta}_k\Big) \bigg| \geq \alpha \max_{\bm{\theta}_k \in \Theta_n}\, \bigg |\frac{\operatorname{d}\! \mathcal{J}}{\operatorname{d} \!\Omega}\Big(\Omega_n\, \Big|\, \bm{\theta}_k\Big) \bigg| = \alpha \, E_n^{\text{mod}}(\Omega_n),
\end{equation}
where $\Theta_n$ contains all the considered directions of differentiation. \\
As an alternative to \eqref{eq:selection_criterion}, we may also consider 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Refine}\label{subsec:algo_refine}
\noindent The purpose of the refinement step is to translate the marked $\beta^+ \in \mathcal{D}^+_{\text{bdry}}$, cf.~\eqref{eq:selection_criterion}, to an appropriate dyadic refinement of boundary elements $Q \in \mathcal{Q}_n$. Upon performing the refinement $\mathcal{Q}_n \rightarrow \mathcal{Q}_{n+1}$, the associated canonical THB-spline basis should:
\begin{itemize}
    \item contain additional boundary degrees of freedom (DOFs) on segments of $\partial \widehat{\Omega}$ where the marked basis functions in $\mathcal{D}_{\text{bdry}}^+$ suggest a large impact on the cost function evaluation can be expected;
    \item Avoid over- and under-refinement.
\end{itemize}
Here, over-/under-refinement is to be understood in the following ways: 1) providing too few additional local DOFs to accurately capture required local changes upon refitting the boundary contours; 2) introducing more additional DOFs than strictly necessary to reach the convergence threshold~\eqref{eq:convergence_criterion}; and 3) accidentally performing element refinement that has no effect on the enriched THB-spline basis. Clearly, a reasonable starting point is defining the set 
$$\mathcal{Q}^+ = \bigcup \limits_{\mathclap{\beta^+ \in \mathcal{D}^+_{\text{bdry}}}} \left\{ Q^+ \in \mathcal{Q}_n^+ \, \vert \, Q^+ \subseteq \operatorname{supp}\left(\beta^+ \right) \right \}$$
and refining all $Q \in \mathcal{Q}_n$ that partially overlap with the $Q^+ \in \mathcal{Q}^+$. This selection ensures that upon refinement, for all $Q^+ \in \left(\mathcal{Q}_n^+ \cap \mathcal{Q}^+ \right)$, we have $Q^+ \in \mathcal{Q}_{n+1}$. Hereby, over- and under-refinement is avoided by suitably choosing the parameter $\alpha \in (0, 1)$. It should be noted that this method may produce elements $Q \in \left(\mathcal{Q}_{n+1} \cap \mathcal{Q}_n^+ \right)$ with $Q \notin \mathcal{Q}^+$ (see Figure \ref{fig:slight_over_refinement}), however, this effect is mild and thus deemed acceptable.
\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{defeaturing_shape_der/img/refine/slight_overrefine_elements_highlighted.png}
    \caption{The $Q \in \mathcal{Q}^+$ highlighted in $\mathcal{Q}_n^+$ (red) and the overlapping elements from $\mathcal{Q}_n$ (blue).}
\end{subfigure} $\quad$
\begin{subfigure}[t]{0.45 \textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{defeaturing_shape_der/img/refine/slight_overrefine_elements_final.png}
    \caption{Illustration of the slight over-refinement in $\mathcal{Q}_{n+1}$.}
\end{subfigure}
\caption{Figure that illustrates the slight over-refinement resulting from refining all $Q \in \mathcal{Q}_n$ that overlap with $\mathcal{Q}^+$.}
\label{fig:slight_over_refinement}
\end{figure}


\noindent A more critical unwanted effect is introducing elements $Q \in \mathcal{Q}^+$ that have no effect on the underlying basis cardinality and hence serve no purpose. For an example, see Figure \ref{fig:over_refinement}.

\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{defeaturing_shape_der/img/refine/overrefine_elements_highlighted.png}
    \caption{The $Q \in \mathcal{Q}^+$ highlighted in on top of $\mathcal{Q}_n$ (red) and the overlapping elements from $\mathcal{Q}_n$ (blue).}
\end{subfigure} $\quad$
\begin{subfigure}[t]{0.45 \textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{defeaturing_shape_der/img/refine/overrefine_elements_final.png}
    \caption{Illustration of over-refinement in $\mathcal{Q}_{n+1}$. The highlighted elements do not impact the basis cardinality.}
\end{subfigure}
\caption{Figure that illustrates how refining all $Q \in \mathcal{Q}_n$ that intersect with $\mathcal{Q}^+$ can produce redundant elements.}
\label{fig:over_refinement}
\end{figure}

\noindent To avoid redundant refinements, in the following, we introduce the concept of \textit{minimal refinement}. As a first step, we define $\mathcal{Q}_{\text{A}}: \mathcal{D}_{\text{bdry}}^+ \rightarrow \mathbb{P} \left(\mathcal{Q}_n \right)$ and $\mathcal{L}_{0}: \mathbb{P}(\mathcal{Q}_n) \rightarrow \mathbb{N}_0$, wherein $\mathbb{P} \left( \cdot \right)$ denotes the power set, with
\begin{align}
    \mathcal{Q}_{\text{A}}\left(\beta^+ \right) = \left \{ Q \in \mathcal{Q}_n \enskip \vert \enskip Q \cap \operatorname{supp}\left(\beta^+ \right) \neq \emptyset \right \} \quad \text{and} \quad \mathcal{L}_{0} \left(\mathcal{Q} \right) = \min \left\{\ell \enskip \vert \enskip Q \in (\mathcal{Q} \cap \mathcal{Q}_\ell) \right \}.
\end{align}
From this, we define the related map
\begin{align}
    \mathcal{Q}_{\text{A}}^\tau \left( \beta^+ \right) = \mathcal{Q}_{\text{A}}(\beta^+) \cap \mathcal{Q}_{\mathcal{L}_0(\mathcal{Q}_{\text{A}}(\beta^+))}
\end{align}
which, in words, removes from $\mathcal{Q}_{\text{A}}(\beta^+)$ all elements whose level in the element hierarchy does not equal the lowest level of the set. Minimal refinement then refines the set of elements
\begin{align}
\label{eq:min_refinement}
    \mathcal{Q}_{\text{min}} = \bigcup \limits_{\mathclap{\beta^+ \in \mathcal{D}_{\text{bdry}}^+}} \mathcal{Q}_{\text{A}}(\beta^+).
\end{align}
For an illustration of how minimal refinement avoids redundant refinements, see Figure \ref{fig:min_refinement}.
\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{defeaturing_shape_der/img/refine/minrefine_elements_highlighted.png}
    \caption{Supporting elements of one $\beta \in \mathcal{D}_{\text{bdry}}^+$ (red) along with the $Q \in \mathcal{Q}_{\text{A}}\left(\beta \right)$ (blue).}
\end{subfigure} $\quad$
\begin{subfigure}[t]{0.45 \textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{defeaturing_shape_der/img/refine/minrefine_elements_final.png}
    \caption{Minimal refinement does not introduce redundant elements.}
\end{subfigure}
\caption{Figure that illustrates how minimal refinement avoids redundant refinements.}
\label{fig:min_refinement}
\end{figure}

\noindent \emph{[Explanation why this works forthcoming]}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation}
This section combines the
\begin{center}
    SOLVE $\rightarrow$ ESTIMATE $\rightarrow$ MARK $\rightarrow$ REFINE.
\end{center}
strategies introduced in Sections \ref{subsec:algo_solve} - \ref{subsec:algo_refine} into an autonomously-operating defeaturing algorithm. As input the algorithm takes the exact boundary correspondence $\mathbf{F}: \partial \widehat{\Omega} \rightarrow \partial \Omega$, the quantity of interest $\mathcal{J}(\, \cdot \,)$, a coarse initial subdivision $\mathcal{Q}_0$ of $\widehat{\Omega}$, the defeaturing tolerance $\epsilon \in \mathbb{R}^+$ and the selection parameter $\alpha \in (0, 1)$. \\

\noindent In each iteration, the first step approximates the exact correspondence $\mathbf{F}$ over the boundary DOFs of the current THB-spline basis $\mathcal{T}_n$ associated with the current subdivision $\mathcal{Q}_n$ which is initialised to $\mathcal{Q}_0$ in the first iteration. Minimisation of~\eqref{eq:boundary_fit} yields the approximate correspondence $\mathbf{F}_n$ which is then forwarded to the parameterisation routine from section \ref{sect:EGG} to compute the mapping \smash{$\mathbf{x}_n: \widehat{\Omega} \rightarrow \Omega_n$}, while performing a posteriori (aPos) refinement if necessary. Hereby, we initialise the parameterisation routine's element subdivision to the current $\mathcal{Q}_n$ plus the previous iteration's refinements (if applicable). This significantly reduces the required number of aPos refinements until a valid map is found. As a next step, we pick suitable element subdivision and basis pairs $(\mathcal{Q}_n^u, \mathcal{T}_n^u)$ and $(\mathcal{Q}_n^p, \mathcal{T}_n^p)$ for the approximation of $u_h$ and $p_h$ of the current geometry's state- and adjoint-equations. Instead of making this choice explicitly, at this point we only list a number of requirements:
\begin{itemize}
    \item $(\mathcal{Q}_n^{u}, \mathcal{Q}_n^{p})$ follow from a sequence of hierarchical refinements of $\mathcal{Q}_0$.
    \item $(u_h, p_h)$ are suitable approximations for accurately computing the shape derivatives.
    \item The numerical error of approximating $u(\Omega_n) \approx u_h$ does not dominate the geometrical error caused by evaluating $\mathcal{J}(\, \cdot \,)$ in $\Omega_n$ instead of $\Omega$.
\end{itemize}
Concrete basis selection strategies are investigated in Section \ref{sec:numerical}.
Upon acquisition of the state and adjoint approximations $(u_h, p_h)$, we are in the position to approximately evaluate the cost function $\mathcal{J}(\Omega_n) \approx J_n = J(u_h, \Omega_n)$ (cf.~\eqref{eq:J_integral}). \\
As a next step the algorithm refines all boundary elements of the current $\mathcal{Q}_n$ to acquire the refined element / basis pair $(\mathcal{Q}_n^+, \mathcal{T}_n^+)$. The pair is forwarded to the minimisation of~\eqref{eq:boundary_fit} which yields the refined boundary fit $\mathbf{F}_n^+$. The discrepancy $\Delta \mathbf{F}_n = \mathbf{F}_n^+ - \mathbf{F}_n$ is expressed in the linear span of $\widetilde{T}_n^+ \subset \mathcal{T}_n^+$ and the associated control points are utilised to define the directions of differentiation $\boldsymbol{\Theta}_n$. With $\boldsymbol{\Theta}_n, u_h$ and $p_h$ at hand, we assemble the approximate shape gradient 
$$\frac{\mathrm{d} \mathcal{J}}{\mathrm{d} \Omega_n} = \left \{ \frac{\mathrm{d} L}{\mathrm{d} \Omega}\big(u_h, p_h; \Omega_n \big \vert \boldsymbol{\theta}_k \big) \, \big \vert \, \boldsymbol{\theta}_k \in \boldsymbol{\Theta}_n \right\},$$
cf.~\eqref{eq:shape_gradient} and exit the loop in case 
$$E^{\text{mod}}_n = \max \limits_{v_k} \left \{ | v_k | \, \vert \, v_k \in \tfrac{\partial \mathcal{J}}{\partial \Omega_n} \right \} < \varepsilon.$$
If $E_n^{\text{mod}} \geq \varepsilon$, we select the set of active $\beta^+ \in \widetilde{\mathcal{T}}_n^+$ according to~\eqref{eq:selection_criterion} and set $\mathcal{Q}_{n+1}$ to the subdivision acquired upon refining all $Q \in \mathcal{Q}_n$ with $Q \in \mathcal{Q}_{\text{min}}$ and move to the next iteration of the loop. \\
All steps are summarised in the pseudocode from Algorithm \ref{algo:simplification}. The algorithm has been implemented in the open-source finite element library \textit{Nutils} \cite{nutils7}.

\begin{algorithm}
	\caption{}
	\label{algo:simplification}
	\small{
	\begin{algorithmic}[1]
		
		\Procedure{Construct simplified geometry $\Omega_S$}{exact correspondence $\mathbf{F}: \partial \widehat{\Omega} \rightarrow \Omega$, functional $\mathcal{J}$, coarse initial mesh $\mathcal{Q}_0$, tolerance $\varepsilon$, selection parameter $\alpha$}
		\Statex
		\For{$n = 0, 1, \ldots$}
		\State $\mathcal{T}_n \longleftarrow$ canonical THB-spline basis associated with $\mathcal{Q}_n$.
		\State $\mathbf{F}_n \longleftarrow$ best approximation of $\mathbf{F}$ over $\widetilde{\mathcal{T}}_n \subset \mathcal{T}_n$ that follows from minimizing~\eqref{eq:boundary_fit}.
		\State $\mathbf{x}_n \longleftarrow$ harmonic map of $\Omega_n$ acquired by solving the Newton scheme~\eqref{eq:EGG_discretized_newton} with Dirichlet data $\mathbf{F}_n$.
		\State $\left( \mathcal{Q}_n^u, \mathcal{T}_n^u \right) \longleftarrow$ element subdivision and THB-spline basis tuple used to solve for $u_h$.
		\State $\left( \mathcal{Q}_n^p, \mathcal{T}_n^p \right) \longleftarrow$ element subdivision and THB-spline basis tuple used to solve for $p_h$.
		\State $(u_h, p_h) \longleftarrow$ discretised weak state- and adjoint equation solutions over $\mathcal{T}_n^u$ and $\mathcal{T}_n^p$, respectively. \Comment{Solve}
		\State $J_n \longleftarrow$ cost function evaluation that results from substituting $(u_h, \Omega_n)$ in~\eqref{eq:J_integral}.
		\State $(\mathcal{Q}_n^+, \mathcal{T}_n^+) \longleftarrow$ element subdivision and basis acquired upon refining all $Q \in \mathcal{Q}_n$ with $\overline{Q} \cap \partial \widehat{\Omega} \neq \emptyset$.
		\State $\mathbf{F}_n^+ \longleftarrow$ best approximation of $\mathbf{F}$ obtained upon minimizing~\eqref{eq:boundary_fit} over $\widetilde{\mathcal{T}}^+_n$.
		\State \smash{$\left\{ \Delta \mathbf{c}_i \right\}_{i = 1}^{\partial N^+} \longleftarrow$} set of control points that follows from expressing $\Delta \mathbf{F}_n = \mathbf{F}_n^+ - \mathbf{F}_n$ in $\operatorname{span} \widetilde{\mathcal{T}}^+_n$.
		\State $\boldsymbol{\Theta}_n \longleftarrow$ directions of differentiation associated with \smash{$\left\{ \Delta \mathbf{c}_i \beta_i^+ \right\}_{i = 1}^{\partial N^+}$}.
		\State $\tfrac{\mathrm{d} \mathcal{J}}{\mathrm{d} \Omega_n} \longleftarrow$ approximate shape gradient resulting from substituting $(u_h, p_h)$ and the \smash{$\boldsymbol{\theta}_k \in \boldsymbol{\Theta}_n$} in~\eqref{eq:shape_gradient}.
		\Statex
		\If{$E^{\text{mod}}_n = \max \limits_{\mathbf{v}_k} \left \{ \left \| \mathbf{v}_k \right \| \, \vert \, \mathbf{v}_k \in \tfrac{\partial \mathcal{J}}{\partial \Omega_n} \right \} < \varepsilon$}
		    \Return{$\Omega_S = \Omega_n$.} \Comment{Estimate}
		\EndIf
		\Statex
		\State $\mathcal{D}_{\text{bdry}}^+ \longleftarrow$ set of active $\beta^+ \in \widetilde{\mathcal{T}}_n^+$ according to \eqref{eq:selection_criterion}. \Comment{Mark}
		\State $\mathcal{Q}_{n+1} \longleftarrow$ new element subdivision acquired upon refining all $Q \in \mathcal{Q}_{\text{min}}$ according to~\eqref{eq:min_refinement}. \Comment{Refine}
		\Statex
		\EndFor
		\EndProcedure{}
		
	\end{algorithmic}
	}
\end{algorithm}

\subsection{Computational aspects}
This section briefly addresses the computational aspects and subtleties associated with Algorithm \ref{algo:simplification} which, so far, have not played a significant role conceptually but require attention in the implementation. \\
Algorithm \ref{algo:simplification} is associated with a total of five element / basis pairs $(\mathcal{Q}_n, \mathcal{T}_n)$

==> intro_backup.tex <==

\textcolor{red}{ we would like to enrich the space to create more and more complex geometries by selecting a set of functions to add, so that the error on the functional decreases. We define an estimator of the modelling error. We consider only changes in the boundary, not topological changes. \\
Say what we mean by exact boundary (spline model or mathematical representation).\\
%DEFINE modelling error (change name?) and defeaturing problem/process (change name wrt Ondine?)
Compared to Ondine, her defeaturing is local, while ours is global.} \\
%We tested only the 2D, but the algorithm can be extended to the 3D provided we have an efficient mesher\\}\\

% Domanda: nel problem setting metto solo neumann BC oppure anche dirichlet? In teoria solo Neumann, pensando al problema vero, ma poi nei test abbiamo anche Dirichlet.

\subsection{Problem setting}
\label{subsec:pb_setting}


\noindent In this work, we focus on the defeaturing problem for two dimensional geometries. Let $\Omega \subset \R^2$ be an open bounded Lipschitz domain with a piecewise smooth, complex boundary. Moreover, let us denote by $U$ the \emph{universe set} of the problem at hand, that is, the collection of all the admissible bounded domains we may consider in the simplification process.\\
\noindent As a model problem defined on the exact geometry $\Omega$, we consider the following scalar elliptic equation, equipped with suitable boundary conditions on $\Gamma_N, \Gamma_D \subset \partial \Omega$ such that $\Gamma_N \cup \Gamma_D = \partial\Omega$ and $\Gamma_N \cap \Gamma_D = \emptyset$:
\begin{equation}
\label{eq:strong_state_pb}
\mathcal{P}(\Omega): \begin{cases} 
- \Delta u &= f \qquad \text{in} \ \Omega, \\
u   &= 0 \qquad \text{on} \ \Gamma_D, \\
\nabla u \cdot \mathbf{n} &= g \qquad \text{on} \ \Gamma_N, \\
\end{cases}
\end{equation}
where $\mathbf{n}$ denotes the unit outward normal to $\Omega$. Similarly, given a simplified domain $\Omega_S \subset \R^2$, $\Omega_S \in U$, we introduce the model problem on the simplified geometry:
\begin{equation}
\label{eq:strong_state_pb_simplified}
\mathcal{P}(\Omega_S): \begin{cases} 
- \Delta u &= f \qquad \text{in} \ \Omega_S, \\
u   &= 0 \qquad \text{on} \ \Gamma_{D}, \\
\nabla u \cdot \mathbf{n}_S &= g \qquad \text{on} \ \Gamma_{N}, \\
\end{cases}
\end{equation}
where now $\Gamma_{N}, \Gamma_{D} \subset \partial \Omega_S$ are such that $\Gamma_{N} \cup \Gamma_{D} = \partial\Omega_S$ and $\Gamma_{N} \cap \Gamma_{D} = \emptyset$, and $\mathbf{n}_S$ denotes the unit outward normal to $\Omega_S$.\\ With a slight abuse of notation, we employ the same letter $u$ for the solutions, and the same symbols $\Gamma_N, \ \Gamma_D$ for the Neumann and Dirichlet boundaries of the two problems. In the following, we will explicitly write their dependence on the domain of definition when needed.\\
%We assume that the Dirichlet boundary $\Gamma_D$ must belong to a portion of the boundary that is fixed and not affected by the defeaturing process; otherwise, indeed, one must define a suitable extension of the datum $h$ for the problem to be well posed on a simplified domain. 
For the data $f \in L^2(\R^2)$ and $g\in H^1(\R^2)$, the weak forms of the two problems read: find $u \in H_{0, \Gamma_D}^1(\Omega)$ such that  
\begin{equation}
\label{eq:weak_state_pb}
    a(u,v \,; \Omega) = b(v \,; \Omega) \qquad \forall \ v \in H_{0, \Gamma_D}^1(\Omega),
\end{equation}
for $\mathcal{P}(\Omega)$; find $u \in H_{0, \Gamma_{D}}^1(\Omega_S)$ such that  
\begin{equation}
\label{eq:weak_state_pb_simplified}
    a(u,v \,; \Omega_S) = b(v \,; \Omega_S) \qquad \forall \ v \in H_{0, \Gamma_{D}}^1(\Omega_S),
\end{equation}
for $\mathcal{P}(\Omega_S)$, where
\begin{equation}
    a(u,v \, ; B) \vcentcolon = \int_{B} \nabla u \cdot \nabla v \operatorname{d}\!\mathbf{x} \quad \text{and} \quad b(v\, ; B) = \int_{B} fv \operatorname{d}\!\mathbf{x} + \int_{\Gamma_N} g v \operatorname{d}\!x.
\end{equation}

\noindent As mentioned before \textcolor{red}{(to do)}, we are interested in computing a functional $J \vcentcolon H_{0, \Gamma_D}^1(\Omega) \rightarrow \R$ of the solution to the problem $\mathcal{P}(\Omega)$. In practice, we are only able to compute the corresponding quantity on the simplified geometry $\Omega_S$, which, therefore, must be wisely chosen to minimize the error in the quantity of interest. 




%that takes the general form:
%\begin{equation}
%\label{eq:form_functionalsJ}
%    J(u) = \int_{\Omega} j(u)\operatorname{d}\!\mathbf{x} \qquad \text{or} \qquad  J(u) = \int_{\partial \Omega}q(u) \operatorname{d}\!x,
%\end{equation} where $ j \vcentcolon H^1(U) \rightarrow L^1(U)$ and $ q \vcentcolon H^1(U) \rightarrow H^1(U)$ \textcolor{red}{OLD: $q \vcentcolon H^{\frac{1}{2}}(\partial \Omega) \rightarrow L^1(\partial \Omega)$} have locally Lipschitz continuous derivative. 

% dire che rendo esplicita la dipendenza da omega per poter valutare l'errore di modello.
\noindent  In order to define the modelling error that we want to estimate and control, it is useful to explicitly write the dependence of $J$ on the geometry. Indeed, not only is $J$ given by an integral on (a part of) $\Omega$ or its boundary, but the integrand itself also depends on the geometry, since $\Omega$ is the domain of definition of the boundary value problem~\eqref{eq:strong_state_pb} solved by $u$. \\%\textcolor{red}{say that the non linearity enters here? is it true?} \\

\noindent To this aim, we introduce some notation that will be used throughout the paper (see Section~\ref{subsec:shapeder} in particular).\\
Let $\mathbb{J} \vcentcolon U \rightarrow \{H^1(B)^*\ | \ B \in U\}$, where $H^1(B)^*$ denotes the dual space of $H^1(B)$, be such that
\begin{equation}
    \begin{aligned}
        \mathbb{J}(B) \vcentcolon H^1(B) &\rightarrow \R \\
        w &\mapsto [\,\mathbb{J}(B)\,](w) \vcentcolon = J(w\,; B).
    \end{aligned}
\end{equation}
In our case, for any element $w$ of $H^1(B)$, the functional $J$ will take the general form 
$$ J(w\,; B) = \int_{B} j\big(w\big)\operatorname{d}\!\mathbf{x} \qquad \text{or}\qquad J(w\,; B)=\int_{\partial B}q\big(w\big) \operatorname{d}\!x,$$
where $ j \vcentcolon H^1(\R^2) \rightarrow L^1(\R^2)$ and $ q \vcentcolon H^1(\R^2) \rightarrow H^1(\R^2)$ %\textcolor{red}{OLD: $q \vcentcolon H^{\frac{1}{2}}(\partial B) \rightarrow L^1(\partial B)$} 
have locally Lipschitz continuous derivatives. \\
Finally, we define the \emph{shape functional} $\mathcal{J} \vcentcolon U \rightarrow \R$ as
\begin{equation}
\label{eq:def_shapefuncJ} 
\mathcal{J}(B) \vcentcolon = [\,\mathbb{J}(B)\,]\big(u(B)\big) = J\big(u(B)\,; B\big), 
\end{equation}
where $u(B)$ is the unique weak solution of $\mathcal{P}(B)$, the model problem~\eqref{eq:strong_state_pb} defined on $B$.\\

%\noindent In the same way, given a simplified domain $\Omega_S \subset U$, we consider the shape functional $\mathcal{J}(\Omega_S) = J\big(u(\Omega_S), \Omega_S \big)$, where $u(\Omega_S)$ is now the exact solution of $\mathcal{P}(\Omega_S)$, that is, of the model problem~\eqref{eq:strong_state_pb} defined on the simplified geometry. \\
\noindent Hence, what we call the modelling error due to the simplification of the geometry is the quantity: 
\begin{equation}
\label{eq:modelling_err}
\abs{\mathcal{J}(\Omega) - \mathcal{J}(\Omega_S)}.
\end{equation}

\begin{remark}
In most cases the functional of interest $\mathcal{J}(\Omega)$ will be an integral over a subdomain $\omega \subset \Omega$ or over a portion of the boundary $\gamma \subset \partial \Omega$. Therefore, we ensure that $\omega \subset \Omega_S$ and $\gamma \subset \partial \Omega_S$ for any simplified geometry $\Omega_S$ we may construct. In this way, we can always compute the error \eqref{eq:modelling_err} and the simplification problem is well defined.
\end{remark}

==> intro_backup2.tex <==

\textcolor{red}{ we would like to enrich the space to create more and more complex geometries by selecting a set of functions to add, so that the error on the functional decreases. We define an estimator of the modelling error. We consider only changes in the boundary, not topological changes. \\
Say what we mean by exact boundary (spline model or mathematical representation).\\
%DEFINE modelling error (change name?) and defeaturing problem/process (change name wrt Ondine?)
Compared to Ondine, her defeaturing is local, while ours is global.} \\
%We tested only the 2D, but the algorithm can be extended to the 3D provided we have an efficient mesher\\}\\

% Domanda: nel problem setting metto solo neumann BC oppure anche dirichlet? In teoria solo Neumann, pensando al problema vero, ma poi nei test abbiamo anche Dirichlet.

\subsection{Problem setting}
\label{subsec:pb_setting}


\noindent In this work, we focus on the defeaturing problem for two dimensional geometries. Let $\Omega \subset \R^2$ be an open bounded Lipschitz domain with a piecewise smooth, complex boundary. Moreover, let us denote by $U$ the \emph{universe set} of the problem at hand, that is, the collection of all the admissible bounded domains $B \subset \mathbb{R}^2$ we may consider in the simplification process.\\
\noindent As a model problem defined on the exact geometry $\Omega$, we consider the following scalar elliptic equation, equipped with suitable boundary conditions on $\Gamma_N, \Gamma_D \subset \partial \Omega$ such that $\Gamma_N \cup \Gamma_D = \partial\Omega$ and $\Gamma_N \cap \Gamma_D = \emptyset$:
\begin{equation}
\label{eq:strong_state_pb}
\mathcal{P}(\Omega): \begin{cases} 
- \Delta u &= f \qquad \text{in} \ \Omega, \\
u   &= 0 \qquad \text{on} \ \Gamma_D, \\
\nabla u \cdot \mathbf{n} &= g \qquad \text{on} \ \Gamma_N, \\
\end{cases}
\end{equation}
where $\mathbf{n}$ denotes the unit outward normal to $\Omega$. Similarly, given a simplified domain $\Omega_S \subset \R^2$, $\Omega_S \in U$, we introduce the model problem on the simplified geometry:
\begin{equation}
\label{eq:strong_state_pb_simplified}
\mathcal{P}(\Omega_S): \begin{cases} 
- \Delta u &= f \qquad \text{in} \ \Omega_S, \\
u   &= 0 \qquad \text{on} \ \Gamma_{D}, \\
\nabla u \cdot \mathbf{n}_S &= g \qquad \text{on} \ \Gamma_{N}, \\
\end{cases}
\end{equation}
where now $\Gamma_{N}, \Gamma_{D} \subset \partial \Omega_S$ are such that $\Gamma_{N} \cup \Gamma_{D} = \partial\Omega_S$ and $\Gamma_{N} \cap \Gamma_{D} = \emptyset$, and $\mathbf{n}_S$ denotes the unit outward normal to $\Omega_S$.\\ 
With a slight abuse of notation, we employ the same letter $u$ for the solutions, and the same symbols $\Gamma_N, \ \Gamma_D$ for the Neumann and Dirichlet boundaries of the two problems. In the following, we will explicitly write their dependence on the domain of definition when needed.\\
%We assume that the Dirichlet boundary $\Gamma_D$ must belong to a portion of the boundary that is fixed and not affected by the defeaturing process; otherwise, indeed, one must define a suitable extension of the datum $h$ for the problem to be well posed on a simplified domain. 
For the data $f \in L^2(\R^2)$ and $g\in H^1(\R^2)$, the weak form of $\mathcal{P}(B)$, with $B \in U$, is based on the problem: \\
\begin{equation}
\label{eq:weak_state_pb}
    \text{Find } u \in H_{0, \Gamma_D}^1(B) \quad \text{s.t.} \quad a(u,v \,; B) = b(v \,; B) \quad \forall \ v \in H_{0, \Gamma_D}^1(B),
\end{equation}
with
\begin{equation}
    a(u,v \, ; B) \vcentcolon = \int_{B} \nabla u \cdot \nabla v \operatorname{d}\!\mathbf{x} \quad \text{and} \quad b(v\, ; B) = \int_{B} fv \operatorname{d}\!\mathbf{x} + \int_{\Gamma_N} g v \operatorname{d}\!x.
\end{equation}
The weak forms of problems~\eqref{eq:strong_state_pb} and~\eqref{eq:strong_state_pb_simplified} then follow from taking $B = \Omega$ and $B = \Omega_S$, respectively. \\

\noindent As mentioned before \textcolor{red}{(to do)}, we are interested in computing a functional $J \vcentcolon H_{0, \Gamma_D}^1(\Omega) \rightarrow \R$ of the solution to the problem $\mathcal{P}(\Omega)$. In practice, we are only able to compute the corresponding quantity on the simplified geometry $\Omega_S$, which, therefore, must be wisely chosen to minimize the error in the quantity of interest. 




%that takes the general form:
%\begin{equation}
%\label{eq:form_functionalsJ}
%    J(u) = \int_{\Omega} j(u)\operatorname{d}\!\mathbf{x} \qquad \text{or} \qquad  J(u) = \int_{\partial \Omega}q(u) \operatorname{d}\!x,
%\end{equation} where $ j \vcentcolon H^1(U) \rightarrow L^1(U)$ and $ q \vcentcolon H^1(U) \rightarrow H^1(U)$ \textcolor{red}{OLD: $q \vcentcolon H^{\frac{1}{2}}(\partial \Omega) \rightarrow L^1(\partial \Omega)$} have locally Lipschitz continuous derivative. 

% dire che rendo esplicita la dipendenza da omega per poter valutare l'errore di modello.
\noindent  In order to define the modelling error that we wish to estimate and control, it is useful to explicitly write the dependence of $J(w)$ on the geometry, i.e., $J(w) \rightarrow J(w \, ; B)$. Indeed, not only is $J(w \,; \Omega)$ given by an integral on (a part of) $\Omega$ or its boundary, but the integrand itself also depends on the geometry, since $\Omega$ is the domain of definition of the boundary value problem~\eqref{eq:strong_state_pb} solved by $u$. \\%\textcolor{red}{say that the non linearity enters here? is it true?} \\

% \noindent To this aim, we introduce some notation that will be used throughout the paper (see Section~\ref{subsec:shapeder} in particular).\\
% Let $\mathbb{J} \vcentcolon U \rightarrow \{H^1(B)^*\ | \ B \in U\}$, where $H^1(B)^*$ denotes the dual space of $H^1(B)$, be such that
% \begin{equation}
%     \begin{aligned}
%         \mathbb{J}(B) \vcentcolon H^1(B) &\rightarrow \R \\
%         w &\mapsto [\,\mathbb{J}(B)\,](w) \vcentcolon = J(w\,; B).
%     \end{aligned}
% \end{equation}
\noindent In our case, for any element $w \in H^1(B)$, the functional $J$ takes the general form 
\begin{equation}
\label{eq:J_integral}
    J(w\,; B) = \int_{B} j\big(w\big)\operatorname{d}\!\mathbf{x} + \int_{\partial B}q\big(w\big) \operatorname{d}\!x,
\end{equation}
where $ j \vcentcolon H^1(\R^2) \rightarrow L^1(\R^2)$ and $ q \vcentcolon H^1(\R^2) \rightarrow H^1(\R^2)$ %\textcolor{red}{OLD: $q \vcentcolon H^{\frac{1}{2}}(\partial B) \rightarrow L^1(\partial B)$} 
have locally Lipschitz continuous derivatives. \\
Finally, we define the \emph{shape functional} $\mathcal{J} \vcentcolon U \rightarrow \R$ as
\begin{equation}
\label{eq:def_shapefuncJ} 
\mathcal{J}(B) \vcentcolon = J\big(u(B)\,; B\big), 
\end{equation}
where $u(B)$ is the unique weak solution of $\mathcal{P}(B)$, the model problem~\eqref{eq:strong_state_pb} defined on $B$.\\

%\noindent In the same way, given a simplified domain $\Omega_S \subset U$, we consider the shape functional $\mathcal{J}(\Omega_S) = J\big(u(\Omega_S), \Omega_S \big)$, where $u(\Omega_S)$ is now the exact solution of $\mathcal{P}(\Omega_S)$, that is, of the model problem~\eqref{eq:strong_state_pb} defined on the simplified geometry. \\
\noindent Hence, what we call the modelling error due to the simplification of the geometry is the quantity: 
\begin{equation}
\label{eq:modelling_err}
\abs{\mathcal{J}(\Omega) - \mathcal{J}(\Omega_S)}.
\end{equation}

\begin{remark}
In most cases, $j(\, \cdot \,)$ and $q(\, \cdot \,)$ in~\eqref{eq:J_integral} will be nonvanishing only over a subdomain $\omega \subset \Omega$ or over a portion of the boundary $\gamma \subset \partial \Omega$, respectively. Therefore, we ensure that $\omega \subset \Omega_S$ and $\gamma \subset \partial \Omega_S$ for any simplified geometry $\Omega_S$ we may construct. In this way, we can always compute the error \eqref{eq:modelling_err} and the simplification problem is well defined.
\end{remark}
